RaidaR: A Rich Annotated Image Dataset of Rainy Street Scenes

We introduce RaidaR, a rich annotated image dataset of rainy street scenes, to support autonomous driving research. The new dataset contains the largest number of rainy images (58,542) to date, 5,000 of which provide semantic segmentations and 3,658 provide object instance segmentations. The RaidaR images cover a wide range of realistic rain-induced artifacts, including fog, droplets, and road reflections, which can effectively augment existing street scene datasets to improve data-driven machine perception during rainy weather. To facilitate efficient annotation of a large volume of images, we develop a semi-automatic scheme combining manual segmentation and an automated processing akin to cross validation, resulting in 10-20 fold reduction on annotation time. We demonstrate the utility of our new dataset by showing how data augmentation with RaidaR can elevate the accuracy of existing segmentation algorithms. We also present a novel unpaired image-to-image translation algorithm for adding/removing rain artifacts, which directly benefits from RaidaR.

==> table_RW.tex <==
% \begin{table}
%   \centering
%   \caption{Comparing popular road datasets and the availability of 2D segmentation of rainy images.  * Weather labels were not originally available on segmented test data. Therefore, a manual evaluation of weather information was necessary for this subset.
%   ** Only front camera frames considered. Weather labels were not originally available, the values shown here were manually curated in the context of this work.}
%   \label{tab:datasets}
%   \begin{threeparttable}
% %   \begin{tabular}{l|c c c c c}
% \textbf{ Name}             & \textbf{Size} & \textbf{Annotated} & \textbf{Rainy} & \textbf{Annotated Rainy}       & \textbf{Type} \\ \hline
% Raincouver                          & 54k           & 326                & 326            & 326                                  & video        \\ %\hline
% BDD                                 & 120M          & 10k                & 5808           & 256 + (83)\tnote{*} & video        \\ %\hline
% nuImages\tnote{**} & 18k           & 1.9k               & 1.3k           & 58                                   & video        \\ %\hline
% Cityscapes                          & 20k           & 20k                & 0              & 0                                    & image        \\ %\hline
% KITTI                               & 15k           & 400                & 0              & 0                                    & video        \\ %\hline
% Apolloscape                                 & 147k          & 147k                & 0           & 0 & video        \\ %\hline
% Ours                                & 77k           & \jc{7k}                  & 58k            & \jc{5k}                                    & video        \\ 
% \end{tabular}
%   \end{threeparttable}
% \end{table}

\setlength\tabcolsep{3pt} % default value: 6pt
\begin{table}
  \centering
      \small
  \begin{threeparttable}
  \begin{tabular}{l|r r r r}
%  \begin{tabular}{m{0.09\textwidth}|m{0.09\textwidth} m{0.05\textwidth} m{0.05\textwidth} m{0.05\textwidth}}
\textbf{ Name}             & \textbf{\#Lab/\#Total} & \textbf{\#Rainy} & \textbf{\#SSeg} & \textbf{\#ISeg}      
\\ \hline
Raincouver~\cite{raincouver}                & 326/54K           & 326            & 326                       & 0                 \\ %\hline
BDD~\cite{BDD}                          & 10K/120M         & 5,808         & 253 & 253       \\ %\hline
nuImages~\cite{caesar2020nuscenes}\tnote{*}   & 1.9K/18K          & 1.3K           & 58       & 58                                   \\ %\hline
Cityscapes~\cite{cityscapes}                & 5K/20K            & 0               & 0         & 0                                 \\ %\hline
KITTI~\cite{Geiger2012CVPR}                       & 400/15K            &  0               & 0        & 0                                  \\ %\hline
Apolloscape~\cite{huang2019apolloscape}             & 147K/147K        &  0                & 0       & 0 \\ %\hline
RID~\cite{li2019single}             & 2.5K/2.5K        &    2.5K              & 0       & 0 \\ %\hline
RaidaR                      & 9K/77K          & \bf 58,542  & \bf 5,000 & \bf 3,658                                        \\ 
\end{tabular}
  \end{threeparttable}
  \caption{Comparing the availability of rainy samples, and their annotations, from well-known street scene image datasets to RaidaR.
\#Lab/\#Total is the ratio between the number of labelled images (rain or no rain) and the total number of images in the datasets; \#Rainy is the number of rainy images; \#SSeg is the number of {\em rainy\/} images with semantic segmentations; and \#ISeg is the number of rainy images with instance segmentations.
%* Manual evaluation of weather information was performed as weather labels were not originally available on segmented test data.
  * Only front camera frames are considered. Weather labels were not originally available, the values shown here are manually curated.}    
    \label{tab:datasets}
\end{table}

